A strong He II $\lambda$1640 emitter with extremely blue UV spectral slope at $z=8.16$: presence of Pop III stars?

Cosmic hydrogen reionization and cosmic production of first metals are major phase transitions of the universe occurring during the first billion years after the Big Bang, however these are still underexplored observationally. Using the JWST NIRSpec prism spectroscopy, we report the discovery of a sub-$L_\ast$ galaxy at $z_{\rm spec}=8.1623\pm0.0007$, dubbed RXJ2129-z8HeII, via the detection of a series of strong rest-frame UV/optical nebular emission lines and the clear Lyman break. RXJ2129-z8HeII shows a pronounced UV continuum with an extremely steep (i.e. blue) spectral slope of $\beta=-2.53_{-0.07}^{+0.06}$, the steepest amongst all spectroscopically confirmed galaxies at $z_{\rm spec}\gtrsim7$, in support of its very hard ionizing spectrum that could lead to a significant leakage of its ionizing flux. Therefore, RXJ2129-z8HeII is representative of the key galaxy population driving the cosmic reionization. More importantly, we detect a strong He II $\lambda$1640 emission line in its spectrum, one of the highest redshifts at which such a line is robustly detected. Its high rest-frame equivalent width (${\rm EW}=21\pm4$ Angstrom) and extreme flux ratios with respect to UV metal and Balmer lines raise the possibility that part of RXJ2129-z8HeII's stellar populations could be Pop III-like. Through careful photoionization modeling, we show that the physically calibrated phenomenological models of the ionizing spectra of Pop III stars with strong mass loss can successfully reproduce the emission line flux ratios observed in RXJ2129-z8HeII. Assuming the Eddington limit, the total mass of the Pop III stars within this system is estimated to be $7.8\pm1.4\times10^5 M_\odot$. To date, this galaxy presents the most compelling case in the early universe where trace Pop III stars might coexist with metal-enriched populations.

==> journals.tex <==
\newcommand{\actaa}{Acta Astron.}   % Acta Astronomica
\newcommand{\araa}{Annu. Rev. Astron. Astrophys.}   % Annual Review of Astron and Astrophys
\newcommand{\areps}{Annu. Rev. Earth Planet. Sci.} % Annual Review of Earth and Planetary Science
\newcommand{\aar}{Astron. Astrophys. Rev.} % Astrononmy and Astrophysics Review
\newcommand{\ab}{Astrobiol.}    % Astrobiology
\newcommand{\aj}{Astron. J.}   % Astronomical Journal
\newcommand{\ac}{Astron. Comput.} % Astronomy and Computing
\newcommand{\apart}{Astropart. Phys.} % Astroparticle Physics
\newcommand{\apj}{Astrophys. J.}   % Astrophysical Journal
\newcommand{\apjl}{Astrophys. J. Lett.}   % Astrophysical Journal, Letters
\newcommand{\apjs}{Astrophys. J. Suppl. Ser.}   % Astrophysical Journal, Supplement
\newcommand{\ao}{Appl. Opt.}   % Applied Optics
\newcommand{\apss}{Astrophys. Space Sci.}   % Astrophysics and Space Science
\newcommand{\aap}{Astron. Astrophys.}   % Astronomy and Astrophysics
\newcommand{\aapr}{Astron. Astrophys. Rev.}   % Astronomy and Astrophysics Reviews
\newcommand{\aaps}{Astron. Astrophys. Suppl.}   % Astronomy and Astrophysics, Supplement
\newcommand{\baas}{Bull. Am. Astron. Soc.}   % Bulletin of the AAS
\newcommand{\caa}{Chin. Astron. Astrophys.}   % Chinese Astronomy and Astrophysics
\newcommand{\cjaa}{Chin. J. Astron. Astrophys.}   % Chinese Journal of Astronomy and Astrophysics (now RAA)
\newcommand{\cqg}{Class. Quantum Gravity}    % Classical and Quantum Gravity
\newcommand{\epsl}{Earth Planet. Sci. Lett.}    % Earth and Planetary Science Letters
\newcommand{\frass}{Front. Astron. Space Sci.}    % Frontiers in Astronomy and Space Sciences
\newcommand{\gal}{Galaxies}    % Galaxies
\newcommand{\gca}{Geochim. Cosmochim. Acta}   % Geochimica Cosmochimica Acta
\newcommand{\grl}{Geophys. Res. Lett.}   % Geophysics Research Letters
\newcommand{\icarus}{Icarus}   % Icarus
\newcommand{\jcap}{J. Cosmol. Astropart. Phys.}   % Journal of Cosmology and Astroparticle Physics
\newcommand{\jgr}{J. Geophys. Res.}   % Journal of Geophysics Research
\newcommand{\jgrp}{J. Geophys. Res.: Planets}    % Journal of Geophysics Research: Planets
\newcommand{\jqsrt}{J. Quant. Spectrosc. Radiat. Transf.} % Journal of Quantitiative Spectroscopy and Radiative Transfer
\newcommand{\lrca}{Living Rev. Comput. Astrophys.}    % Living Reviews in Computational Astrophysics
\newcommand{\lrr}{Living Rev. Relativ.}    % Living Reviews in Relativity
\newcommand{\lrsp}{Living Rev. Sol. Phys.}    % Living Reviews in Solar Physics
\newcommand{\memsai}{Mem. Soc. Astron. Italiana}   % Mem. Societa Astronomica Italiana
\newcommand{\mnras}{Mon. Not. R. Astron. Soc.}   % Monthly Notices of the RAS
\newcommand{\nat}{Nature} % Nature
\newcommand{\nastro}{Nat. Astron.} % Nature Astronomy
\newcommand{\ncomms}{Nat. Commun.} % Nature Communications
\newcommand{\nphys}{Nat. Phys.} % Nature Physics
\newcommand{\na}{New Astron.}   % New Astronomy
\newcommand{\nar}{New Astron. Rev.}   % New Astronomy Review
\newcommand{\physrep}{Phys. Rep.}   % Physics Reports
\newcommand{\pra}{Phys. Rev. A}   % Physical Review A: General Physics
\newcommand{\prb}{Phys. Rev. B}   % Physical Review B: Solid State
\newcommand{\prc}{Phys. Rev. C}   % Physical Review C
\newcommand{\prd}{Phys. Rev. D}   % Physical Review D
\newcommand{\pre}{Phys. Rev. E}   % Physical Review E
\newcommand{\prl}{Phys. Rev. Lett.}   % Physical Review Letters
\newcommand{\psj}{Planet. Sci. J.}   % Planetary Science Journal
\newcommand{\planss}{Planet. Space Sci.}   % Planetary Space Science
\newcommand{\pnas}{Proc. Natl Acad. Sci. USA}   % Proceedings of the US National Academy of Sciences
\newcommand{\procspie}{Proc. SPIE}   % Proceedings of the SPIE
\newcommand{\pasa}{Publ. Astron. Soc. Aust.}   % Publications of the Astron. Soc. of Australia
\newcommand{\pasj}{Publ. Astron. Soc. Jpn}   % Publications of the Astron. Soc. of Japan (note no full stop following Jpn)
\newcommand{\pasp}{Publ. Astron. Soc. Pac.}   % Publications of the Astron. Soc. of the Pacific
\newcommand{\raa}{Res. Astron. Astrophys.} % Research in Astronomy and Astrophysics (formerly CJAA)
\newcommand{\rmxaa}{Rev. Mexicana Astron. Astrofis.}   % Revista Mexicana de Astronomia y Astrofisica
\newcommand{\sci}{Science} % Science
\newcommand{\sciadv}{Sci. Adv.} % Science Advances
\newcommand{\solphys}{Sol. Phys.}   % Solar Physics
\newcommand{\sovast}{Soviet Astron.}   % Soviet Astronomy
\newcommand{\ssr}{Space Sci. Rev.}   % Space Science Reviews
\newcommand{\uni}{Universe} % Universe

